Defensive Adversarial CAPTCHA: A Semantics-Driven Framework for Natural Adversarial Example Generation

Traditional CAPTCHA (Completely Automated Public Turing Test to Tell Computers and Humans Apart) schemes are increasingly vulnerable to automated attacks powered by deep neural networks (DNNs). Existing adversarial attack methods often rely on the original image characteristics, resulting in distortions that hinder human interpretation and limit their applicability in scenarios where no initial input images are available. To address these challenges, we propose the Unsourced Adversarial CAPTCHA (DAC), a novel framework that generates high-fidelity adversarial examples guided by attacker-specified semantics information. Leveraging a Large Language Model (LLM), DAC enhances CAPTCHA diversity and enriches the semantic information. To address various application scenarios, we examine the white-box targeted attack scenario and the black box untargeted attack scenario. For target attacks, we introduce two latent noise variables that are alternately guided in the diffusion step to achieve robust inversion. The synergy between gradient guidance and latent variable optimization achieved in this way ensures that the generated adversarial examples not only accurately align with the target conditions but also achieve optimal performance in terms of distributional consistency and attack effectiveness. In untargeted attacks, especially for black-box scenarios, we introduce bi-path unsourced adversarial CAPTCHA (BP-DAC), a two-step optimization strategy employing multimodal gradients and bi-path optimization for efficient misclassification. Experiments show that the defensive adversarial CAPTCHA generated by BP-DAC is able to defend against most of the unknown models, and the generated CAPTCHA is indistinguishable to both humans and DNNs.

==> coverlatter.tex <==
Cover Letter

Editorial Office
IEEE Transactions on Dependable and Secure Computing
Dear Editor,

I am pleased to submit our manuscript titled “Defensive Adversarial CAPTCHA: A Semantics-Driven Framework for Natural Adversarial Example Generation” for consideration in IEEE Transactions on Dependable and Secure Computing. This work is original, has not been published elsewhere, and is not under review by any other publication, the main contribution for our work are summarized below:

Summary of the Work
Our work proposes an innovative framework called Defensive Adversarial CAPTCHA (DAC) to address the issues of insufficient diversity, copyright restrictions, and weak adversarial robustness faced by traditional CAPTCHAs due to their reliance on original images to generate adversarial examples. The core of this framework is to generate adversarial CAPTCHAs without requiring source images through semantic-driven generation, combined with large language models (LLMs) to enhance semantic diversity and accuracy. It also designs a Bi-path optimization strategy tailored for different attack scenarios:
1: White-box target attack scenario: Proposes a coupling latent noise variable optimization mechanism based on a diffusion model, which generates high-fidelity adversarial examples through alternating gradient guidance and latent variable calibration to ensure attack accuracy and image quality.
2: Black-box untarget attack scenario: We propose a Bi-path DAC (BP-DAC) strategy that integrates multi-model gradients and adopts dual-path optimization (simultaneously optimizing suboptimal category and target category gradients), significantly improving the transfer attack success rate of adversarial examples on unknown models.
Experiments show that DAC-generated captchas outperform traditional methods in both human readability and adversarial robustness, achieving efficient adversarial captcha generation without requiring source images for the first time.

Precision targeting: The work achieves high-precision control through semantics-driven methods in white-box attack scenarios, with the core mechanism being the coupling of latent noise variable optimization. By constructing parameter-shared noise variable pairs within the diffusion model and utilizing the EDICT framework for dynamic bidirectional calibration, this mechanism alternates between gradient backpropagation and variable updates at each diffusion step, effectively reducing error accumulation. This design ensures that adversarial examples are strictly aligned with the target semantics, achieving a high attack success rate on DNN models. At the same time, detailed semantic prompts generated by large language models (LLMs) ensure semantic consistency, and the generated CAPTCHAs are far more user-friendly than traditional adversarial CAPTCHA methods.

Enhanced adversarial transferability: For unknown model attacks in black-box scenarios, the paper proposes the BP-DAC strategy, which significantly improves transfer generalization capabilities. This strategy first integrates the prediction probability distributions of three proxy models through multi-model gradient aggregation to generate weighted adversarial gradients, thereby expanding the attack coverage. It then employs a dual-path optimization engine to simultaneously minimize the loss of the target category and the loss of the suboptimal category, forcing the unknown black-box model to produce confusion at the decision boundary and breaking through the generalization bottleneck of traditional diffusion-based adversarial attack methods.

Robust reversibility: This work establishes a robust balance between defensive robustness and human usability, ensuring stable deployment of anti-CAPTCHA systems in harsh environments. On one hand, defense against cracking is achieved through dual-path optimization: under four mainstream defense preprocessing methods, it still maintains a high attack success rate, far exceeding other diffusion-based adversarial attack methods. The core lies in the adaptive disturbance of the decision boundary through gradient aggregation strategies. On the other hand, human readability is achieved by constraining the semantic space using the CLIP model to achieve a high Clip Score.

Relevance to the Journal
This work proposes the Defensive Adversarial CAPTCHA (DAC) framework to directly address key cybersecurity challenges. Through semantics-driven adversarial example generation, it breaks through the copyright and diversity limitations of traditional CAPTCHAs that rely on raw images, significantly improving the dependability of the system's defense against automated attacks. In response to cutting-edge adversarial defense issues, the designed dual-path optimization strategy (BP-DAC) achieves a high transfer attack success rate in black-box scenarios and ensures that the generated samples maintain high robustness under defensive preprocessing through a gradient coupling mechanism, which is highly consistent with TDSC's research focus on new adversarial defense technologies and transfer attacks.

Corresponding Author
Dr. Jizhe Zhou
Engineering Research Center of Machine Learning and Industry Intelligence 
Sichuan University 
Chengdu, 610020, China
Email: yb87409@um.edu.mo

Thank you for considering our submission. We look forward to your feedback.

Sincerely,
Xia Du, Xiaoyuan Liu, Jizhe Zhou, Zheng Lin, Chi-man Pun, Cong Wu, Tao Li, Zhe Chen, Wei Ni, Jun Luo

